The Mini-CAPTAIN Liquid Argon Time Projection Chamber

This manuscript describes the commissioning of the Mini-CAPTAIN liquid argon detector in a neutron beam at the Los Alamos Neutron Science Center (LANSCE), which led to a first measurement of high-energy neutron interactions in argon. The Mini-CAPTAIN detector consists of a Time Projection Chamber (TPC) with an accompanying photomultiplier tube (PMT) array sealed inside a liquid-argon-filled cryostat. The liquid argon is constantly purified and recirculated in a closed-loop cycle during operation. The specifications and assembly of the detector subsystems and an overview of their performance in a neutron beam are reported.

==> simulation.tex <==
$<$... Insert description of simulated track reconstruction... $>$

Work continues on track reconstruction from the neutron run.

\subsection{Simulation Mode}
\subsection{Track Reconstruction}

